A Discontinuity Adjustment for Subdistribution Function Confidence Bands Applied to Right-Censored Competing Risks Data (with Erratum)

The wild bootstrap is the resampling method of choice in survival analytic applications. Theoretic justifications rely on the assumption of existing intensity functions which is equivalent to an exclusion of ties among the event times. However, such ties are omnipresent in practical studies. It turns out that the wild bootstrap should only be applied in a modified manner that corrects for altered limit variances and emerging dependencies. This again ensures the asymptotic exactness of inferential procedures. An analogous necessity is the use of the Greenwood-type variance estimator for Nelson-Aalen estimators which is particularly preferred in tied data regimes. All theoretic arguments are transferred to bootstrapping Aalen-Johansen estimators for cumulative incidence functions in competing risks. An extensive simulation study as well as an application to real competing risks data of male intensive care unit patients suffering from pneumonia illustrate the practicability of the proposed technique.

==> EP10_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 87.72 & 88.64 & 89.37 & 90.69 & 89.87 & 90.84 \\ 
   & 75 & 89.22 & 90.16 & 91.86 & 92.55 & 91.75 & 92.35 \\ 
   & 100 & 90.68 & 91.22 & 92.43 & 93.07 & 93.06 & 93.31 \\ 
   & 125 & 91.13 & 91.61 & 93.05 & 93.50 & 93.42 & 93.79 \\ 
  25\% & 150 & 91.63 & 92.16 & 93.5 & 93.77 & 93.48 & 93.79 \\ 
   & 175 & 91.79 & 92.06 & 93.87 & 94.19 & 93.75 & 93.93 \\ 
   & 200 & 91.93 & 92.37 & 93.84 & 93.94 & 93.70 & 93.88 \\ 
   & 225 & 92.40 & 92.77 & 93.54 & 93.89 & 93.73 & 93.97 \\ 
   & 250 & 92.17 & 92.61 & 94.03 & 94.26 & 94.24 & 94.56 \\ \hline
   & 50 & 87.15 & 88.59 & 89.20 & 90.73 & 89.18 & 90.50 \\ 
   & 75 & 89.78 & 90.80 & 91.46 & 92.47 & 91.18 & 92.22 \\ 
   & 100 & 90.24 & 91.32 & 92.58 & 93.25 & 92.53 & 93.47 \\ 
   & 125 & 91.17 & 92.11 & 92.99 & 93.70 & 93.06 & 93.76 \\ 
  50\% & 150 & 91.63 & 92.52 & 93.25 & 93.98 & 93.17 & 93.95 \\ 
   & 175 & 92.65 & 93.29 & 92.67 & 93.34 & 93.06 & 93.71 \\ 
   & 200 & 92.21 & 92.87 & 93.36 & 94.03 & 93.51 & 94.23 \\ 
   & 225 & 92.20 & 92.98 & 94.07 & 94.80 & 93.09 & 93.96 \\ 
   & 250 & 92.96 & 93.52 & 93.71 & 94.23 & 93.37 & 93.93 \\ \hline
   & 50 & 87.63 & 89.82 & 89.19 & 91.41 & 88.95 & 90.91 \\ 
   & 75 & 89.52 & 91.46 & 91.97 & 93.42 & 91.36 & 92.96 \\ 
   & 100 & 90.30 & 91.90 & 92.45 & 93.76 & 92.52 & 93.95 \\ 
   & 125 & 91.44 & 92.88 & 92.93 & 94.03 & 92.83 & 94.14 \\ 
  75\% & 150 & 91.49 & 92.76 & 93.20 & 94.50 & 93.22 & 94.23 \\ 
   & 175 & 91.50 & 92.76 & 92.98 & 94.18 & 93.66 & 94.63 \\ 
   & 200 & 92.00 & 93.08 & 93.92 & 94.94 & 93.75 & 94.85 \\ 
   & 225 & 92.20 & 93.12 & 93.57 & 94.56 & 93.17 & 94.13 \\ 
   & 250 & 92.49 & 93.78 & 93.51 & 94.55 & 93.69 & 94.81 \\ \hline
   & 50 & 88.28 & 91.10 & 90.21 & 92.75 & 90.31 & 92.68 \\ 
   & 75 & 89.81 & 92.2 & 91.70 & 93.90 & 91.77 & 93.57 \\ 
   & 100 & 90.54 & 92.66 & 92.10 & 93.98 & 92.09 & 93.96 \\ 
   & 125 & 91.12 & 93.19 & 92.58 & 94.36 & 92.74 & 94.47 \\ 
  100\% & 150 & 91.41 & 93.44 & 92.83 & 94.61 & 92.77 & 94.77 \\ 
   & 175 & 91.60 & 93.59 & 92.84 & 94.57 & 92.84 & 94.79 \\ 
   & 200 & 91.49 & 93.46 & 93.03 & 94.76 & 93.25 & 94.97 \\ 
   & 225 & 92.32 & 93.98 & 92.92 & 94.70 & 93.38 & 94.95 \\ 
   & 250 & 91.81 & 93.81 & 92.79 & 94.58 & 92.98 & 94.73 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of equal precision bands in per cent where $k=10$} 
\label{tab:EP10}
\end{table}


==> EP20_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 87.21 & 88.03 & 89.93 & 90.94 & 90.15 & 90.69 \\ 
   & 75 & 89.75 & 90.33 & 92.18 & 92.50 & 91.78 & 92.38 \\ 
   & 100 & 91.01 & 91.61 & 93.12 & 93.52 & 92.71 & 93.08 \\ 
   & 125 & 92.09 & 92.29 & 93.99 & 94.18 & 93.34 & 93.67 \\ 
  25\% & 150 & 91.87 & 92.39 & 93.63 & 93.78 & 93.69 & 93.85 \\ 
   & 175 & 92.44 & 92.71 & 94.03 & 94.40 & 94.19 & 94.35 \\ 
   & 200 & 92.76 & 93.03 & 94.18 & 94.35 & 93.76 & 94.07 \\ 
   & 225 & 93.23 & 93.44 & 94.46 & 94.77 & 94.02 & 94.23 \\ 
   & 250 & 92.84 & 93.11 & 93.88 & 94.10 & 94.16 & 94.41 \\ \hline
   & 50 & 88.02 & 89.22 & 89.57 & 90.86 & 89.59 & 90.81 \\ 
   & 75 & 89.88 & 90.74 & 92.37 & 93.28 & 92.34 & 93.00 \\ 
   & 100 & 90.95 & 91.69 & 93.19 & 93.74 & 93.02 & 93.71 \\ 
   & 125 & 91.98 & 92.46 & 93.44 & 93.83 & 93.91 & 94.2 \\ 
  50\% & 150 & 91.90 & 92.54 & 93.60 & 94.01 & 93.97 & 94.27 \\ 
   & 175 & 92.95 & 93.40 & 94.00 & 94.42 & 94.11 & 94.45 \\ 
   & 200 & 92.79 & 93.11 & 94.05 & 94.39 & 93.68 & 94.00 \\ 
   & 225 & 92.78 & 93.25 & 94.16 & 94.53 & 94.28 & 94.67 \\ 
   & 250 & 93.01 & 93.28 & 93.92 & 94.30 & 93.77 & 94.03 \\ \hline
   & 50 & 88.42 & 89.91 & 90.81 & 92.12 & 90.51 & 91.96 \\ 
   & 75 & 90.28 & 91.50 & 92.73 & 93.94 & 92.85 & 93.67 \\ 
   & 100 & 91.43 & 92.45 & 93.30 & 94.21 & 93.02 & 93.85 \\ 
   & 125 & 91.41 & 92.30 & 93.84 & 94.58 & 93.57 & 94.08 \\ 
  75\% & 150 & 92.73 & 93.31 & 94.01 & 94.77 & 93.54 & 94.25 \\ 
   & 175 & 92.44 & 93.14 & 94.44 & 95.04 & 94.09 & 94.82 \\ 
   & 200 & 93.04 & 93.84 & 94.13 & 94.65 & 94.02 & 94.58 \\ 
   & 225 & 93.32 & 93.94 & 94.41 & 94.95 & 94.08 & 94.69 \\ 
   & 250 & 93.03 & 93.59 & 94.27 & 94.85 & 94.29 & 94.77 \\ \hline
   & 50 & 88.87 & 90.73 & 91.04 & 92.79 & 91.16 & 92.69 \\ 
   & 75 & 90.95 & 92.58 & 93.21 & 94.28 & 93.02 & 94.24 \\ 
   & 100 & 91.98 & 93.28 & 93.74 & 95.01 & 93.74 & 94.67 \\ 
   & 125 & 92.91 & 93.94 & 93.69 & 94.88 & 94.13 & 95.13 \\ 
  100\% & 150 & 92.82 & 93.88 & 94.18 & 95.10 & 94.58 & 95.49 \\ 
   & 175 & 93.16 & 94.25 & 94.88 & 95.59 & 94.85 & 95.74 \\ 
   & 200 & 93.53 & 94.51 & 94.38 & 95.30 & 94.59 & 95.29 \\ 
   & 225 & 94.06 & 94.76 & 94.63 & 95.59 & 94.69 & 95.39 \\ 
   & 250 & 93.12 & 94.31 & 94.95 & 95.79 & 94.79 & 95.60 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of equal precision bands in per cent where $k=20$} 
\label{tab:EP20}
\end{table}


==> EP5_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 87.31 & 88.47 & 89.44 & 90.61 & 88.93 & 90.36 \\ 
   & 75 & 89.48 & 90.39 & 91.55 & 92.24 & 91.13 & 92.01 \\ 
   & 100 & 90.64 & 91.26 & 92.32 & 92.96 & 92.21 & 92.64 \\ 
   & 125 & 91.21 & 91.96 & 92.36 & 93.07 & 93.43 & 93.76 \\ 
  25\% & 150 & 91.12 & 91.66 & 92.48 & 92.98 & 93.37 & 93.75 \\ 
   & 175 & 91.69 & 92.14 & 93.10 & 93.21 & 93.20 & 93.63 \\ 
   & 200 & 91.99 & 92.46 & 93.31 & 93.80 & 93.63 & 94.05 \\ 
   & 225 & 92.51 & 92.98 & 93.29 & 93.67 & 93.58 & 94.03 \\ 
   & 250 & 92.48 & 92.88 & 93.65 & 93.91 & 93.41 & 93.84 \\ \hline
   & 50 & 87.41 & 89.31 & 89.09 & 91.28 & 89.76 & 91.29 \\ 
   & 75 & 89.35 & 90.99 & 91.28 & 92.71 & 91.03 & 92.59 \\ 
   & 100 & 90.01 & 91.53 & 92.39 & 93.64 & 91.88 & 93.29 \\ 
   & 125 & 90.56 & 91.92 & 92.95 & 93.90 & 92.29 & 93.43 \\ 
  50\% & 150 & 90.59 & 91.93 & 92.44 & 93.38 & 93.04 & 94.05 \\ 
   & 175 & 91.21 & 92.22 & 92.58 & 93.49 & 92.66 & 93.73 \\ 
   & 200 & 91.22 & 92.28 & 92.30 & 93.31 & 93.16 & 94.19 \\ 
   & 225 & 91.44 & 92.61 & 92.70 & 93.73 & 93.25 & 94.16 \\ 
   & 250 & 91.72 & 92.82 & 93.13 & 94.27 & 93.07 & 94.05 \\ \hline
   & 50 & 87.23 & 90.60 & 89.12 & 91.56 & 89.47 & 92.11 \\ 
   & 75 & 90.09 & 92.56 & 90.96 & 93.22 & 91.29 & 93.77 \\ 
   & 100 & 90.58 & 92.86 & 92.13 & 94.23 & 91.59 & 93.83 \\ 
   & 125 & 90.83 & 93.03 & 92.13 & 94.26 & 91.75 & 94.08 \\ 
  75\% & 150 & 90.84 & 93.11 & 91.96 & 93.94 & 92.29 & 94.35 \\ 
   & 175 & 90.83 & 93.13 & 91.66 & 93.87 & 92.25 & 94.03 \\ 
   & 200 & 90.91 & 93.11 & 92.45 & 94.46 & 92.50 & 94.49 \\ 
   & 225 & 91.15 & 93.43 & 92.52 & 94.49 & 92.22 & 94.12 \\ 
   & 250 & 91.76 & 93.76 & 92.38 & 94.36 & 92.73 & 94.53 \\ \hline
   & 50 & 87.71 & 91.98 & 89.08 & 92.91 & 89.56 & 93.19 \\ 
   & 75 & 88.79 & 92.70 & 90.26 & 93.74 & 90.21 & 93.64 \\ 
   & 100 & 89.89 & 93.25 & 90.90 & 94.06 & 90.47 & 93.84 \\ 
   & 125 & 89.76 & 93.14 & 90.92 & 93.88 & 90.44 & 93.64 \\ 
  100\% & 150 & 89.64 & 93.21 & 90.84 & 93.97 & 91.00 & 93.87 \\ 
   & 175 & 90.10 & 93.24 & 90.52 & 93.52 & 91.25 & 93.99 \\ 
   & 200 & 90.27 & 93.55 & 91.06 & 94.00 & 91.09 & 94.12 \\ 
   & 225 & 90.01 & 93.07 & 91.30 & 94.19 & 91.08 & 94.26 \\ 
   & 250 & 89.71 & 93.18 & 90.92 & 93.89 & 90.76 & 93.86 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of equal precision bands in per cent where $k=5$} 
\label{tab:EP5}
\end{table}


==> HW10_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 87.21 & 88.70 & 89.27 & 90.49 & 89.00 & 90.36 \\ 
   & 75 & 89.23 & 90.08 & 90.91 & 91.57 & 90.65 & 91.51 \\ 
   & 100 & 90.54 & 90.86 & 91.86 & 92.55 & 91.40 & 91.89 \\ 
   & 125 & 91.49 & 91.96 & 92.45 & 92.86 & 91.59 & 92.25 \\ 
  25\% & 150 & 92.52 & 92.80 & 92.31 & 92.94 & 92.18 & 92.65 \\ 
   & 175 & 92.61 & 92.88 & 92.86 & 93.06 & 92.71 & 93.23 \\ 
   & 200 & 92.25 & 92.76 & 92.66 & 92.88 & 92.80 & 93.20 \\ 
   & 225 & 92.92 & 93.41 & 93.02 & 93.32 & 93.00 & 93.38 \\ 
   & 250 & 92.37 & 92.78 & 92.90 & 93.29 & 93.19 & 93.46 \\ \hline
   & 50 & 87.32 & 89.05 & 88.85 & 90.49 & 89.17 & 90.77 \\ 
   & 75 & 89.94 & 91.20 & 91.08 & 92.27 & 90.65 & 91.81 \\ 
   & 100 & 91.24 & 92.37 & 91.08 & 92.32 & 91.51 & 92.59 \\ 
   & 125 & 91.05 & 92.16 & 91.61 & 92.49 & 91.88 & 92.77 \\ 
  50\% & 150 & 91.99 & 92.82 & 91.92 & 92.79 & 92.00 & 93.01 \\ 
   & 175 & 92.37 & 93.10 & 92.53 & 93.21 & 92.66 & 93.38 \\ 
   & 200 & 92.24 & 92.79 & 92.42 & 93.37 & 92.59 & 93.25 \\ 
   & 225 & 92.29 & 93.22 & 92.75 & 93.44 & 92.87 & 93.64 \\ 
   & 250 & 92.05 & 92.73 & 92.70 & 93.38 & 92.05 & 92.74 \\ \hline
   & 50 & 88.15 & 90.60 & 88.32 & 91.01 & 89.49 & 91.71 \\ 
   & 75 & 90.41 & 92.20 & 91.34 & 92.98 & 90.39 & 92.28 \\ 
   & 100 & 91.25 & 92.74 & 90.97 & 92.66 & 91.19 & 93.00 \\ 
   & 125 & 91.76 & 93.21 & 91.99 & 93.34 & 91.57 & 93.09 \\ 
  75\% & 150 & 91.67 & 92.85 & 91.73 & 93.04 & 91.90 & 93.31 \\ 
   & 175 & 92.30 & 93.57 & 92.50 & 93.75 & 92.08 & 93.34 \\ 
   & 200 & 92.25 & 93.46 & 92.11 & 93.50 & 92.05 & 93.46 \\ 
   & 225 & 92.40 & 93.63 & 92.43 & 93.88 & 92.89 & 94.09 \\ 
   & 250 & 92.70 & 93.79 & 92.38 & 93.66 & 92.56 & 93.67 \\ \hline
   & 50 & 88.99 & 92.00 & 89.50 & 92.73 & 89.59 & 92.83 \\ 
   & 75 & 91.10 & 93.57 & 91.14 & 93.59 & 90.91 & 93.76 \\ 
   & 100 & 90.84 & 93.12 & 92.10 & 94.27 & 91.66 & 93.77 \\ 
   & 125 & 92.06 & 93.80 & 92.06 & 94.18 & 92.25 & 94.27 \\ 
  100\% & 150 & 91.95 & 93.89 & 92.56 & 94.65 & 92.60 & 94.59 \\ 
   & 175 & 92.41 & 94.23 & 92.87 & 94.70 & 92.27 & 94.35 \\ 
   & 200 & 92.34 & 94.21 & 93.11 & 94.88 & 92.99 & 94.88 \\ 
   & 225 & 92.73 & 94.31 & 93.25 & 94.85 & 93.06 & 94.89 \\ 
   & 250 & 93.32 & 94.90 & 92.74 & 94.41 & 92.90 & 94.61 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of Hall-Wellner bands in per cent where $k=10$} 
\label{tab:HW10}
\end{table}


==> HW20_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 88.39 & 89.53 & 89.93 & 91.16 & 89.14 & 90.05 \\ 
   & 75 & 90.39 & 90.99 & 90.67 & 91.39 & 90.74 & 91.52 \\ 
   & 100 & 91.39 & 91.89 & 91.75 & 92.26 & 91.92 & 92.30 \\ 
   & 125 & 91.69 & 92.17 & 92.54 & 93.03 & 92.52 & 92.90 \\ 
  25\% & 150 & 92.07 & 92.51 & 92.57 & 92.83 & 92.92 & 93.28 \\ 
   & 175 & 92.24 & 92.55 & 92.76 & 92.97 & 92.8 & 93.07 \\ 
   & 200 & 93.01 & 93.27 & 92.58 & 93.04 & 92.96 & 93.21 \\ 
   & 225 & 93.11 & 93.32 & 92.99 & 93.25 & 93.16 & 93.42 \\ 
   & 250 & 92.88 & 93.03 & 93.60 & 93.69 & 93.05 & 93.31 \\ \hline
   & 50 & 88.77 & 90.02 & 89.28 & 90.66 & 89.53 & 90.89 \\ 
   & 75 & 90.43 & 91.37 & 91.27 & 92.29 & 90.87 & 91.92 \\ 
   & 100 & 91.74 & 92.45 & 91.99 & 92.74 & 91.94 & 92.62 \\ 
   & 125 & 92.12 & 92.82 & 92.49 & 93.11 & 92.08 & 92.61 \\ 
  50\% & 150 & 92.12 & 92.59 & 93.05 & 93.60 & 92.56 & 93.18 \\ 
   & 175 & 92.43 & 93.00 & 92.96 & 93.25 & 93.00 & 93.45 \\ 
   & 200 & 92.94 & 93.22 & 93.08 & 93.50 & 92.69 & 93.28 \\ 
   & 225 & 92.67 & 93.01 & 93.20 & 93.92 & 93.51 & 93.90 \\ 
   & 250 & 93.41 & 93.58 & 93.03 & 93.47 & 92.74 & 93.25 \\ \hline
   & 50 & 89.17 & 90.83 & 89.70 & 91.53 & 89.65 & 91.36 \\ 
   & 75 & 90.99 & 92.23 & 91.29 & 92.41 & 91.21 & 92.32 \\ 
   & 100 & 91.15 & 92.12 & 92.36 & 93.24 & 92.26 & 93.37 \\ 
   & 125 & 92.21 & 93.15 & 92.57 & 93.44 & 92.49 & 93.50 \\ 
  75\% & 150 & 92.64 & 93.39 & 93.08 & 93.98 & 92.68 & 93.46 \\ 
   & 175 & 92.50 & 93.21 & 93.25 & 93.91 & 92.67 & 93.44 \\ 
   & 200 & 92.73 & 93.39 & 93.34 & 94.15 & 93.10 & 93.78 \\ 
   & 225 & 92.91 & 93.51 & 93.18 & 93.96 & 93.61 & 94.11 \\ 
   & 250 & 93.34 & 94.01 & 93.84 & 94.39 & 92.92 & 93.67 \\ \hline
   & 50 & 90.11 & 92.25 & 90.74 & 92.78 & 90.52 & 92.90 \\ 
   & 75 & 91.22 & 92.70 & 92.57 & 94.08 & 91.94 & 93.44 \\ 
   & 100 & 92.01 & 93.62 & 93.09 & 94.37 & 92.49 & 93.84 \\ 
   & 125 & 92.39 & 93.45 & 93.28 & 94.64 & 93.59 & 94.56 \\ 
  100\% & 150 & 92.77 & 94.10 & 93.47 & 94.59 & 93.28 & 94.41 \\ 
   & 175 & 93.22 & 94.35 & 93.66 & 94.84 & 94.00 & 94.93 \\ 
   & 200 & 93.88 & 94.73 & 93.79 & 94.78 & 93.90 & 94.84 \\ 
   & 225 & 93.74 & 94.62 & 94.25 & 95.07 & 93.69 & 94.70 \\ 
   & 250 & 93.61 & 94.56 & 93.94 & 94.95 & 94.17 & 95.12 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of Hall-Wellner bands in per cent where $k=20$} 
\label{tab:HW20}
\end{table}


==> HW5_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:50 2017
\begin{table}[ht]
\centering
\begin{tabular}{c|c|cc|cc|cc}
  \multicolumn{2}{c|}{set-ups} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird}  \\ \hline
  $p$ & $n$ & old & new & old & new & old & new \\ \hline
   & 50 & 88.65 & 89.93 & 89.33 & 90.79 & 88.85 & 90.18 \\ 
   & 75 & 89.82 & 90.60 & 90.59 & 91.54 & 90.39 & 91.32 \\ 
   & 100 & 90.51 & 91.11 & 90.93 & 91.82 & 91.13 & 91.88 \\ 
   & 125 & 90.92 & 91.69 & 91.11 & 91.82 & 91.07 & 91.92 \\ 
  25\% & 150 & 91.41 & 91.70 & 91.53 & 92.20 & 92.21 & 92.74 \\ 
   & 175 & 91.79 & 92.17 & 92.75 & 93.17 & 92.65 & 93.16 \\ 
   & 200 & 92.24 & 92.67 & 92.18 & 92.59 & 92.26 & 92.73 \\ 
   & 225 & 92.22 & 92.70 & 92.75 & 93.20 & 92.64 & 93.14 \\ 
   & 250 & 92.38 & 93.03 & 92.53 & 93.05 & 92.44 & 92.68 \\ \hline
   & 50 & 87.72 & 90.36 & 88.52 & 90.87 & 88.77 & 91.14 \\ 
   & 75 & 89.17 & 91.06 & 89.54 & 91.43 & 89.92 & 91.87 \\ 
   & 100 & 89.86 & 91.62 & 90.26 & 91.87 & 90.60 & 92.18 \\ 
   & 125 & 90.86 & 92.28 & 91.27 & 92.69 & 91.00 & 92.39 \\ 
  50\% & 150 & 90.99 & 92.28 & 91.34 & 92.77 & 91.15 & 92.57 \\ 
   & 175 & 91.41 & 92.67 & 91.76 & 92.84 & 91.12 & 92.42 \\ 
   & 200 & 91.77 & 92.99 & 92.20 & 93.57 & 91.78 & 92.86 \\ 
   & 225 & 91.70 & 92.87 & 91.72 & 92.95 & 91.94 & 93.14 \\ 
   & 250 & 91.44 & 92.84 & 92.00 & 93.20 & 91.65 & 93.04 \\ \hline
   & 50 & 87.35 & 90.83 & 88.74 & 92.14 & 88.32 & 91.82 \\ 
   & 75 & 89.97 & 92.41 & 90.57 & 93.39 & 90.09 & 93.16 \\ 
   & 100 & 89.89 & 92.60 & 90.32 & 93.29 & 90.19 & 93.01 \\ 
   & 125 & 90.52 & 92.98 & 90.95 & 93.38 & 91.03 & 93.55 \\ 
  75\% & 150 & 90.61 & 93.03 & 91.15 & 93.80 & 91.16 & 93.67 \\ 
   & 175 & 91.03 & 93.41 & 91.54 & 93.95 & 90.88 & 93.37 \\ 
   & 200 & 91.29 & 93.53 & 90.98 & 93.49 & 91.30 & 93.41 \\ 
   & 225 & 91.63 & 93.76 & 91.70 & 93.52 & 91.11 & 93.61 \\ 
   & 250 & 91.44 & 93.55 & 91.55 & 93.78 & 91.95 & 94.24 \\ \hline
   & 50 & 88.99 & 92.88 & 89.60 & 93.67 & 89.68 & 93.41 \\ 
   & 75 & 90.32 & 93.74 & 90.71 & 94.31 & 90.23 & 93.99 \\ 
   & 100 & 90.59 & 94.04 & 91.17 & 94.37 & 90.60 & 94.14 \\ 
   & 125 & 91.27 & 94.59 & 91.79 & 94.81 & 91.56 & 94.55 \\ 
  100\% & 150 & 91.63 & 94.59 & 91.42 & 94.50 & 91.20 & 94.60 \\ 
   & 175 & 91.53 & 94.56 & 91.95 & 94.80 & 90.97 & 94.22 \\ 
   & 200 & 91.78 & 94.65 & 91.82 & 94.68 & 91.76 & 94.68 \\ 
   & 225 & 91.94 & 94.92 & 91.87 & 94.81 & 91.59 & 94.56 \\ 
   & 250 & 92.40 & 94.92 & 91.86 & 94.76 & 91.35 & 94.46 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of Hall-Wellner bands in per cent where $k=5$} 
\label{tab:HW5}
\end{table}


==> HWEP0_final.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Fri Jan 27 17:17:35 2017
\begin{table}[H]
\centering
\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
  & \multicolumn{6}{|c|}{Hall-Wellner} &  \multicolumn{6}{|c}{Equal Precision} \\ \hline
  & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c|}{weird} & \multicolumn{2}{c|}{$N(0,1)$} & \multicolumn{2}{c|}{$Poi(1)-1$}  & \multicolumn{2}{c}{weird} \\ \hline
  $n$ & old & new & old & new & old & new & old & new & old & new & old & new \\ \hline
  50 & 87.61 & 88.64 & 88.80 & 90.03 & 88.72 & 89.75 & 87.08 & 88.06 & 89.55 & 90.36 & 89.43 & 90.48 \\ 
  75 & 90.15 & 90.75 & 90.71 & 91.46 & 90.74 & 91.48 & 89.36 & 90.21 & 91.79 & 92.33 & 91.62 & 92.14 \\ 
  100 & 90.78 & 91.31 & 91.13 & 91.58 & 91.77 & 92.23 & 90.74 & 91.24 & 93.20 & 93.43 & 92.43 & 92.72 \\ 
  125 & 91.72 & 92.07 & 92.02 & 92.31 & 91.58 & 92.23 & 91.35 & 91.77 & 92.96 & 93.37 & 93.19 & 93.54 \\ 
  150 & 92.29 & 92.54 & 92.60 & 92.85 & 92.90 & 93.21 & 91.33 & 91.52 & 93.64 & 93.85 & 93.51 & 93.76 \\ 
  175 & 92.27 & 92.53 & 92.48 & 92.83 & 92.86 & 93.17 & 92.45 & 92.64 & 93.91 & 94.14 & 94.06 & 94.39 \\ 
  200 & 92.67 & 92.85 & 92.89 & 93.02 & 93.18 & 93.34 & 92.87 & 93.04 & 93.68 & 93.80 & 93.47 & 93.83 \\ 
  225 & 92.98 & 93.05 & 92.60 & 92.71 & 93.26 & 93.68 & 92.69 & 92.93 & 93.85 & 94.12 & 94.16 & 94.22 \\ 
  250 & 92.78 & 92.99 & 92.93 & 93.14 & 93.14 & 93.32 & 93.20 & 93.43 & 93.68 & 93.81 & 94.25 & 94.30 \\ 
   \hline
\end{tabular}
\caption{Simulated coverage probabilities of confidence bands for $F_1$ in per cent where $p=0$} 
\label{tab:HWEPcont}
\end{table}

